Transactional Indexes on (RDMA or CXL-based) Disaggregated Memory with Repairable Transaction

The failure atomic and isolated execution of clients operations is a default requirement for a system that serve multiple loosely coupled clients at a server. However, disaggregated memory breaks this requirement in remote indexes because a client operation is disaggregated to multiple remote reads/writes. Current indexes focus on performance improvements and largely ignore tolerating client failures. We argue that a practical DM index should be transactional: each index operation should be failure atomic and isolated in addition to being concurrency isolated. We present repairable transaction (rTX), a lightweight primitive to execute DM index operations. Each rTX can detect other failed rTXes on-the-fly with the help of concurrency control. Upon detection, it will repair their non-atomic updates online with the help of logging, thus hiding their failures from healthy clients. By further removing unnecessary logging and delegating concurrency control to existing carefully-tuned index algorithms, we show that transactional indexes can be built at a low performance overhead on disaggregated memory. We have refactored two state-of-the-art DM indexes, RaceHashing and Sherman (B+Tree), with rTX. Evaluations show that rTX is 1.2 to 2X faster than other alternatives, e.g., distributed transaction. Meanwhile, its overhead is up to 42% compared to non-fault-tolerant indexes.

==> ack.tex <==
Mingyu Wu: information about types
Nian Liu: for related works on locks 
Zhiyuan Dong: feedbacks of an early version of the paper
Dingyan for sharing thoughts on LegoOS
Rongxin for evaluating FUSE.

Authors from fuse and sherman for validating performance. 

==> object.tex <==
\section{{\sys} Memory Objects}
\label{sec:memory-obj-api}

\begin{figure}[!t]
\begin{minipage}{1\linewidth}
\hspace{-4mm}
\centering    
\includegraphics[scale=1]{figs/object.pdf}
\end{minipage} \\[5pt]
\begin{minipage}{1\linewidth}
\caption{\small{%
\TODO{XXX: system name not known. xxx: bits }
}}
\label{fig:object}
\end{minipage} \\[-20pt]
\end{figure}

==> overhead-race.tex <==
\begin{table}[t]
%    \vspace{3mm}
    \begin{minipage}{.48\textwidth}
        \caption{\small{
        A summary of the DM operations of inserting an 8\,B value to various {\race} implementations,
        assuming only the directory is cached at the CNs.
        Note that {\rtx} achieves the same \texttt{CAS} as {\race} because we delegate our concurrency control to it.
        }}
        \label{tab:overhead-race}
        \end{minipage} 
        \centering
        \resizebox{.47\textwidth}{!}{%    
        \small{            
    \centering%\small{
        \begin{tabular}{l|ccc}
            \hline
            & \textbf{READ (Bytes)}            & \textbf{WRITE (Bytes)}               & \textbf{CAS (Bytes)} \\ \hline
    \textbf{Optimal} & $40 \times 4 \times 2$               & $8$         & $8$       \\
    \textbf{DTX}     & $(40 + \red{\uline{32}}) \times 4$                   & $8  \red{\uline{\times 2}}$     & $8$       \\
    \textbf{\rtx}     & $(40 + \red{\uline{32}}) \times 4$ + \red{\uline{16}}                   & $8$               & $8 $       \\
            \bottomrule
    \end{tabular}
    
        }

    }
    \end{table}

==> related-far.tex <==
\textbf{Far memory-aware data structures}~\cite{racehashing,rolex, DBLP:conf/sigmod/WangLS22, DBLP:conf/sigmod/0001VBFK19}

==> related-rdma.tex <==
\textbf{RDMA-aware data structures}~\cite{mitchell2013pilaf, farm, DBLP:conf/sosp/WeiSCCC15, farmv2,cell,  xstore} 

==> related-tx.tex <==
\textbf{Far memory-aware distributed transaction}~\cite{farm,farmv2,drtmh,DBLP:conf/sosp/WeiSCCC15,ford-fast22,DBLP:conf/eurosys/ChenWSCC16}

==> relatedtab.tex <==
\begin{table*}[t]  
    \centering    
    \vspace{8pt}  
    \begin{minipage}{1\textwidth}
        \caption{{\small{
        \textbf{Existing solutions (\textsection{\ref{sec:existing-solutions}}). } 
        The columns correspond to our goals summarized in \textsection{\ref{sec:goals}}.
        \textbf{Partial} means the approach can only satisfy a goal in some scenarios (detailed in \textsection{\ref{sec:existing-solutions}}).
        \iffalse
        \textbf{Atomicity} (Failure atomicity), 
        \textbf{HA} (High availability), 
        \textbf{Transparency} (Transparent fault tolerance),
        \textbf{Lightweight} and \textbf{Efficiency}. 
        \fi
        }}}
        \label{tab:motiv-related}
        \end{minipage} %\\[2pt]  
        \ra{1.2}
        \small{            
        \resizebox{.96\textwidth}{!}{%    
        \begin{tabular}{l|ccccc}
            \toprule
                                                        & \textbf{Atomicity}        & \textbf{HA}               & \textbf{Transparency} & \textbf{Lightweight}      & \textbf{Efficiency} \\ \hline
\input{related-rdma.tex}                                & Partial                   &  Partial                  &                       & \checkmark                & \checkmark          \\
\input{related-far.tex}                                 &                           &                           &                       & \checkmark                & \checkmark          \\
%\textbf{Data structures on persistent memory}           & \checkmark                &                           &                      & \checkmark                & \checkmark          \\       
%\textbf{Persistent transactional memory}                & \checkmark                &                           &  \checkmark          & \checkmark                &                     \\
\input{related-tx.tex}                                  & \checkmark                & \checkmark                &  \checkmark           &                           &                     \\
\textbf{\red{{\sys}}} (This work)                       & \checkmark                & \checkmark                &  \checkmark           & \checkmark                & \checkmark          \\
\bottomrule
\end{tabular}
        }
        }
\\[-5pt]
\end{table*}         


==> stm-related.tex <==
STM~\cite{DBLP:conf/eurosys/HermanIHTKLS16,DBLP:conf/pldi/SpiegelmanGK16}
